Property Testing for Ocean Models. Can We Specify It? (Invited Talk)

I take inspiration from the property-testing literature, particularly the work of Prof. John Hughes, and explore how such ideas might be applied to numerical models of the ocean. Specifically, I ask whether geophysical fluid dynamics (GFD) theory, expressed as property tests, might be used to address the oracle problem of testing the correctness of ocean models. I propose that a number of simple idealized GFD problems can be framed as property tests. These examples clearly illustrate how physics naturally lends itself to specifying property tests. Which of these proposed tests might be most feasible and useful, remains to be seen.

==> eptcsdata.tex <==
\providecommand{\firstpage}{48}
\providecommand{\publicationstatus}{S.F.\ Siegel and G.\ Gopalakrishnan (Eds.):\\
International Workshop on Verification of\\
Scientific Software (VSS 2025)\\
EPTCS 432, 2025, pp.\ \pageref*{FirstPage}--\pageref{LastPage},
doi:\href{https://dx.doi.org/10.4204/EPTCS.432.7}{10.4204/EPTCS.432.7}}
\pdfoutput=1

